CorAl: Introspection for Robust Radar and Lidar Perception in Diverse Environments Using Differential Entropy

Robust perception is an essential component to enable long-term operation of mobile robots. It depends on failure resilience through reliable sensor data and preprocessing, as well as failure awareness through introspection, for example the ability to self-assess localization performance. This paper presents CorAl: a principled, intuitive, and generalizable method to measure the quality of alignment between pairs of point clouds, which learns to detect alignment errors in a self-supervised manner. CorAl compares the differential entropy in the point clouds separately with the entropy in their union to account for entropy inherent to the scene. By making use of dual entropy measurements, we obtain a quality metric that is highly sensitive to small alignment errors and still generalizes well to unseen environments. In this work, we extend our previous work on lidar-only CorAl to radar data by proposing a two-stage filtering technique that produces high-quality point clouds from noisy radar scans. Thus we target robust perception in two ways: by introducing a method that introspectively assesses alignment quality, and applying it to an inherently robust sensor modality. We show that our filtering technique combined with CorAl can be applied to the problem of alignment classification, and that it detects small alignment errors in urban settings with up to 98% accuracy, and with up to 96% if trained only in a different environment. Our lidar and radar experiments demonstrate that CorAl outperforms previous methods both on the ETH lidar benchmark, which includes several indoor and outdoor environments, and the large-scale Oxford and MulRan radar data sets for urban traffic scenarios The results also demonstrate that CorAl generalizes very well across substantially different environments without the need of retraining.

==> Journal/abstract.tex <==
\begin{abstract}
%%%%
%This paper presents CorAl, a principled and intuitive measure for alignment quality and self-supervised method method that learns to detect alignment errors. CorAl estimates alignment quality by computing differential entropy in the joint point cloud and in the separate to account for entropy inherent to the scene.
%By making use of dual entropy measurements, we obtain a quality metric, highly sensitive to small alignment errors.
%In this work we extend our previous work by proposing a two-step filtering technique that produces high quality point clouds from noisy radar data. We found that our proposed filtering technique combined CorAl could be applied to the problem of alignment classification, and detect small alignment errors within urban settings with up to 98\% accuracy, and with up to 96\% if trained only on a different environment type. Lidar and radar experiments coherently demonstrate that our method outperform previous methods within a lidar benchmark, within large scale trafficked urban scenarios and enables a high degree of generalization across substantially different environments without need of retraining.
%%%%
%\\{\normalfont{Abstract V2}} %%%
Robust perception is an essential component to enable long-term operation of mobile robots. It depends on failure resilience through reliable sensor data and pre-processing, as well as failure awareness through introspection, for example the abaility to self-assess localization performance.
This paper presents CorAl: a principled, intuitive, and generalizable method to measure the quality of alignment between pairs of point clouds, which learns to detect alignment errors in a self-supervised manner. 
CorAl compares the differential entropy in the point clouds separately with the entropy in their union to account for entropy inherent to the scene.
By making use of dual entropy measurements, we obtain a quality metric that is highly sensitive to small alignment errors and still generalizes well to unseen environments.
In this work, we extend our previous work on lidar-only CorAl to radar data by proposing a two-step filtering technique that produces high-quality point clouds from noisy radar scans.  
Thus we target robust perception in two ways: by introducing a method that introspectively assesses alignment quality, and applying it to an inherently robust sensor modality.
We show that our filtering technique combined with CorAl can be applied to the problem of alignment classification, and that it detects small alignment errors in urban settings with up to 98\% accuracy, and with up to 96\% if trained only in a different environment. 
Our lidar and radar experiments demonstrate that CorAl outperforms previous methods both on the ETH lidar benchmark, which includes several indoor and outdoor environments, and the large-scale Oxford and MulRan radar data sets for urban traffic scenarios
The results also demonstrate that CorAl generalizes very well across substantially different environments without the need of retraining.
%%%%


%In robotics perception, numerous tasks rely on point cloud registration, however registration is not guaranteed fully reliable. However, currently there is no method that can automatically detect misaligned point clouds reliably and without environment-specific parameters. We propose ``CorAl'', an alignment quality measure and alignment classifier for point cloud pairs, which facilitates the ability to introspectively assess the performance of registration and highlight regions containing evidence of misalignment. 
%CorAl compares the joint and the separate entropy of the two point clouds. The separate entropy provides a measure of the entropy given a single point cloud that can be expected to be inherent to the environment. The joint entropy computed from the resulting registered clouds should therefore not be substantially higher if the point clouds are properly aligned.
%Using dual differential entropy measurements makes the method able to detect small alignment errors, which are particularly hard to detect, and applicable in a range of different environments. 
%We found that CorAl is able to detect small alignment errors in previously unseen environments with an accuracy of 95\% and achieve a substantial improvement to previous methods.
\end{abstract}

==> Journal/backup/backup <==
\label{sec:method}
\label{sec:method}



Our work is inspired by the  Mean-Map-Entropy (MME) measure proposed by Droeschel and Behnke~\cite{8461000} for map quality assessment. MME is based on differential entropy~\cite{article} and measures the randomness of multivariate Gaussian distributions. Droeschel and Behnke  used  MME in absence of accurate ground truth when evaluating map refinement.
As shown in our evaluation, MME cannot be used as a general alignment quality measure as it is also affected by measurement noise, sample density and environment geometry. MME is more affected by changes in the environment compared to CorAl. Hence, the measure is not expected to generalize between, e.g., a structured warehouse and an unstructured outdoor forest environment. We  overcome this effect using dual entropy measurements computed 1) in both point clouds separately and 2) in the joint point cloud. The intuition is that joining two well-aligned point clouds should not introduce additional uncertainty and entropy should remain constant if the point clouds overlap sufficiently.
\subsection{Computing joint and separate entropy}


Our method operates on the dense point clouds $\mathcal{P}_a$, $\mathcal{P}_b$, given in a common fixed world frame, that contain a set of points in the Cartesian space $\bold{p}_k=
\begin{bmatrix}
x & y & z
\end{bmatrix}$.
For later use, we define the joint point cloud $\jointPC=\mathcal{P}_a \cup \mathcal{P}_b$; i.e., all points in $\mathcal{P}_a$ and  $\mathcal{P}_b$ together.

From all points within a radius $r$ around each point $\bold{p}_k$, we compute the sample covariance $\bold{\Sigma(p}_k)$. From the determinant of the sample covariance $\det(\bold{\Sigma}(\bold{p}_k))$ we can then compute the differential entropy as:
\begin{equation}
    \label{eqn:point_entropy}
    h_{i}(\bold{p}_k)=\frac{1}{2}\ln(2\pi e\det(\Sigma(\bold{p}_k)))
\end{equation}
for the point cloud $i=a,b$ that contains $\bold{p}_k$. An example of point clouds colored according to \cref{eqn:point_entropy} can be seen in Fig.~\ref{fig:entropy_src} and \ref{fig:entropy_target}.
The sum of differential entropy for $\mathcal{P}_i$ can then be computed as % in eq.\ref{eqn:cloud_etntropy}:
\begin{equation}
    \label{eqn:cloud_etntropy}
    H_i(\mathcal{P}_i)=\sum_{k=1}^{|\mathcal{P}_i|}h_i(\bold{p}_k)
    ,
\end{equation}
where $|\mathcal{P}_i|$ is the number of points in the point cloud $\mathcal{P}_i$. 

Using Eq.~\ref{eqn:cloud_etntropy} we can derive measures of the \emph{separate} and \emph{joint} average differential entropy of two point clouds $\mathcal{P}_a, \mathcal{P}_b$.
\begin{equation}
    \label{eq:Hseparate}
    H_{\mathrm{sep}}=\frac{H_{a}(\mathcal{P}_a)+H_{b}(\mathcal{P}_b)}{|\mathcal{P}_a|+|\mathcal{P}_b|}
    ,
\end{equation}
\begin{equation}
    \label{eq:Hjoint}
    H_{\mathrm{joint}}=\frac{H_j(\mathcal{P}_j)}{|\mathcal{P}_j|}=\frac{H(\mathcal{P}_a\cup\mathcal{P}_b)}{|\mathcal{P}_a|+|\mathcal{P}_b|}
    .
\end{equation}

Our first %proposed
alignment quality measure uses the %average
difference between the joint and the separate average differential entropy:

\begin{equation}
    \label{eqn:EntropyDifference}
    Q(\mathcal{P}_a,\mathcal{P}_b)=H_{\mathrm{joint}}(\mathcal{P}_{j})-H_{\mathrm{sep}}(\mathcal{P}_a,\mathcal{P}_b)
    ,
\end{equation}
%
which can also be given per-point by
\begin{equation}
    \label{eqn:point_quality}
    q_k(\bold{p}_k)=h_{j}(\bold{p}_k)-h_{i}(\bold{p}_k)
    ,
\end{equation}
where the point entropy is evaluated on the joint point cloud $j$ and the separate point cloud $i$ =  ($a$ or $b$) where  $\bold{p}_k$ originates from. An example of point clouds colored by per-point entropy difference according to ~\cref{eqn:point_quality} is depicted in Fig.~\ref{fig:entropy_diff_aligned} and \ref{fig:entropy_diff_misaligned}. Typically, $Q(\mathcal{P}_a,\mathcal{P}_b)$ is close to zero for well-aligned point clouds and increases with the alignment error as depicted in \cref{fig:qualityMeasurePlot}, which visualizes the function's surface for position and angular alignment errors around the correct alignment.
\begin{figure}
\centering
\subfloat[Top view of first two aligned point clouds $\mathcal{P}_a$(blue) and $\mathcal{P}_b$(red) in the ETH ``stairs'' dataset. 
]{\includegraphics[trim={0cm 13cm 3cm 15cm},clip,width=0.99\hsize,angle=0]{figures/other/stairs2.png}%
\label{fig:top_view_stais}}\\
\vspace{-0.2cm}
\subfloat[][\raggedright CorAl measure $Q(\mathcal{P}_a,\mathcal{P}_b)$ \cref{eqn:EntropyDifference} visualized by color for various (x,y) displacements.]{\includegraphics[trim={0.0cm 0cm 0.0cm 0cm},clip,width=0.49\hsize]{Journal/figures/ETH/objective/narrow_position_objective.png}\label{fig:quality_xy_plot}}
\subfloat[][\raggedright CorAl measure $Q(\mathcal{P}_a,\mathcal{P}_b)$ for various (x,$\theta$) displacements.]{\includegraphics[trim={0cm 0cm 0cm 0cm},clip,width=0.49\hsize]{Journal/figures/ETH/objective/narrow_angle_objective.png}\label{fig:quality_xtheta_plot}}
\caption{
Example of CorAl measure $Q(\mathcal{P}_a,\mathcal{P}_b)$ for various induced (x,y,$\theta$) alignment errors.
$Q$ has a minimum at the true position. The steepness of the surface around the true alignment indicates that CorAl is sensitive to small misalignments.
\label{fig:qualityMeasurePlot}}
\vspace{-0.5cm}
\end{figure}

Well-aligned point clouds  $\mathcal{P}_a\cup\mathcal{P}_b$ acquired in structured environments have low differential entropy for most query points $\bold{p}_k$. This is reflected by low values for the determinant of the sample covariance. As the determinant can be expressed as the product of the eigenvalues of the sample covariance $\det(\bold{\Sigma(\bold{p}}_k))=\lambda_1\lambda_2\lambda_3$, we see that the measure is sensitive to an increase in the lowest of the eigenvalues when larger eigenvalues are constant. For example, the entropy of points on a planar surface is represented with a flat distribution with two large ($\lambda_1,\lambda_2$) and one small ($\lambda_3$) eigenvalue. Misalignment changes the point distribution in the joint point cloud from flat to ellipsoidal which can be observed as an increase of the smallest eigenvalue $\lambda_3$. This makes the measure sensitive to misalignment of planar surfaces, but generalizes well to other geometries. As shown in the evaluation, the measure can capture discrepancies between point clouds regardless of whether these are due to rigid misalignments or distortions which can can occur when scanning while moving, e.g. because of vibrations or sensor velocity estimation errors. That means that the method can be overly sensitive when used together with a registration method or odometry framework that does not compensate movement distortion or has a low accuracy.

\begin{figure}
\centering
\subfloat[Aligned point clouds: differential entropy distributions are similar.]{\includegraphics[clip,trim={2.0cm 0cm 2cm 0cm},width=0.49\hsize]{figures/distributions/aligned_distributions2.png}\label{fig:entropy_aligned}}\hfill%
\subfloat[Misaligned point clouds: joint differential entropy is higher.
]{\includegraphics[clip,trim={1.8cm 0cm 1.8cm 0cm},width=0.49\hsize]{figures/distributions/misaligned_distributions2.png}\label{fig:entropy_misaligned}}
\caption{\label{fig:entropypdf}
Probability distribution of per-point entropy \cref{eqn:point_entropy} for joint and separate point clouds when (a) aligned and (b) misaligned. Aligned point clouds have similar joint and separate entropy distributions, while joint entropy is higher compared to separate entropy when point clouds are misaligned.  Joining misaligned point clouds blurs the scene which can be observed by an entropy increase.
An exception can be seen in (a) region $(-12,-8)$ where the entropy increases by joining aligned point clouds.}

\vspace{-0.3cm}
\end{figure}


Overlap is required between point clouds to produce evidence of alignment. For that reason, we classify point clouds with less than 10\% overlap as misaligned. By defining the overlap as all points with a neighbor within $r$ in the other point cloud, non overlapping points have no effect on the quality measure in \cref{eqn:EntropyDifference}.

\subsection{Dynamic radius selection and outlier rejection }

For well aligned point clouds, the quality measure is close to zero, meaning that the joint and separate point clouds have similar mean and probability distributions of per-point entropy as depicted in Fig.~\ref{fig:entropy_aligned}.
Unfortunately, the entropy in \cref{eqn:point_entropy} is ill-posed when the determinant
$\det(\bold{\Sigma}(\bold{p}_k))$ is
close to zero and a small increase of the determinant causes a large increase of the entropy. 
Accordingly, the lowest measured entropies can increase (which indicates misalignment) even when joining well aligned point clouds as depicted in~\cref{fig:entropy_aligned}. 

The ill-posed entropies are found where point density is low, typically for solitary points or far from the sensor where the radius $r$ is not large enough to include points that represent the geometry in the environment. The effect of the problem with entropies can be mitigated by maximizing the ratio $Q_s=Q_{misaligned}(\mathcal{P}_a,\mathcal{P}_b)/Q_{aligned}(\mathcal{P}_a,\mathcal{P}_b)$. A larger ratio indicates that the measure is able to discriminate between aligned and misaligned point clouds.
\begin{figure*}[htb!]
  \begin{center}
    \subfloat[]{\includegraphics[trim={0.0cm 2cm 0cm 0cm},clip,width=0.249\hsize]{figures/orkla/fixed_r_noeps_al.png}\label{fig:settings_a}}\hfill
    \subfloat[]{\includegraphics[trim={0.0cm 2cm 0cm 0cm},clip,width=0.249\hsize]{figures/orkla/fixed_r_eps_al.png}\label{fig:settings_b}}\hfill
    \subfloat[]{\includegraphics[trim={0.0cm 2cm 0cm 0cm},clip,width=0.249\hsize]{figures/orkla/dyn_r_al.png}\label{fig:settings_c}}\hfill
    \subfloat[]{\includegraphics[trim={0.0cm 2cm 0cm 0cm},clip,width=0.249\hsize]{figures/orkla/dyn_r_erej_al.png}\label{fig:settings_d}}\\
    \vspace{-0.2cm}
     \subfloat[]{\includegraphics[trim={0.0cm 2cm 0cm 0cm},clip,width=0.249\hsize]{figures/orkla/fixed_r_noeps_misal.png}\label{fig:settings_e}}\hfill
    \subfloat[]{\includegraphics[trim={0.0cm 2cm 0cm 0cm},clip,width=0.249\hsize]{figures/orkla/fixed_r_eps_misal.png}\label{fig:settings_f}}\hfill
    \subfloat[]{\includegraphics[trim={0.0cm 2cm 0cm 0cm},clip,width=0.249\hsize]{figures/orkla/dyn_r_misal.png}\label{fig:settings_g}}\hfill
    \subfloat[]{\includegraphics[trim={0.0cm 2cm 0cm 0cm},clip,width=0.249\hsize]{figures/orkla/dyn_r_erej_misal.png}\label{fig:settings_h}}
        	\caption{
        	Joint point cloud colored by per-point quality, $q_k$ ranging from blue (aligned) to red (misaligned). The location of the point cloud origin is highlighted in \cref{fig:orkla}.
        	Columns depict the same parameters for aligned (top) and misaligned (bottom) point clouds.  (a,e): A fixed radius $r=0.3m$ gives $(Q_s=1.46)$. (b,f): radius dynamically adjusted $r_{min}=0.3$m,$\alpha=1.33,r_{max}=0.7$ gives $(Q_s=2.93)$. (c,g):  $\epsilon=10^{-8}$ is added $(Q_s=4.06)$. (d,h): $\Ereject=10\%$ is added ($Q_s=4.3$).  
    	 }\label{fig:modifications}
  \end{center}
  \vspace{-0.3cm}
\end{figure*}

We propose three strategies to address the ill-posed entropies due to variations in sampling density originating from the sensor.

(1): Eq.~\ref{eqn:point_entropy} is modified to   $h_{i}(\bold{p}_k)=\frac{1}{2}\ln(2\pi e\det(\bold{\Sigma(p}_k))+\epsilon)$ where $\epsilon$ limits the lowest possible entropy. 
This make sure that entropy is similar for points distributed along a line and a plane.
%The change make sure that points distributed along a line or a plane are assigned similarly high entropy. 
The improvement can be seen by comparing  \cref{fig:modifications}(a-b).

(2): Radius $r$ is chosen based on the distance $d$ between the point $\bold{p}_k$ and the sensor location, to account for that point density decrease over distance. The radius is hence selected as: $r=d \sin(\alpha)$ in the range $r_{min} < r < r_{max}$ where $\alpha$ is the vertical resolution of the sensor. %and is not tuned by the user
For other sensor types e.g. RGB-D, the resolution could be chosen similarly according to the angular sensing resolution.
 A dynamic radius enables the quality measure to include more points far from the sensor and correctly detect alignment and misalignment for these as seen in \cref{fig:modifications}(c).

(3): Remove $\Ereject$ percent of points $\bold{p}_k$ with the lowest entropies.
The effect is depicted in \cref{fig:modifications}(d). 

\subsection{Classification}\label{sec:classifier}
We use logistic regression as a model for classification:
\begin{equation}
\begin{split}
    &p=\frac{1}{1+e^{-z}},\\
    &z=\beta_0+\beta_1x_1+\beta_2x_2\\
\end{split}
\end{equation}

\begin{equation}
    \label{eq:classifier}
       y_{pred}= 
\begin{cases}
  \mathrm{aligned} & \mathrm{if} \: p\geq t_h \\
      \mathrm{misaligned} & \mathrm{if} \: p<t_h,
\end{cases}
\end{equation}
where $x_1,x_2$ are input variables (described for each method in \cref{sec:methods}). 

Instead of passing the quality measure $x_1=Q(\mathcal{P}_a,\mathcal{P}_b)$, $H_{sep}$ and $H_{joint}$ are passed separately to $x_1=H_{joint}$ and $ x_2=H_{sep}$.
$\beta_0,\beta_1,\beta_2$ are learned model parameters, $p$ is the class probability and $t_h$ is a class probability threshold and can be adjusted to the application needs. 
For example, in mobile robotics, it is desired that misaligned point clouds are not accidentally reported as aligned (false positives), potentially causing a system failure. In contrast, aligned point clouds classified as misaligned are typically harmless. For that reason, $t_h$ can be increased to reject false positives and hence improve robustness. We used the default threshold $t_h=0.5$. During training, weights of data points was adjusted inversely proportional to class occurrence to mitigate bias.


\subsection{CorAl For spinning radar}\label{sec:classifier}
Spinning radar produces $360^\circ$ sweep ($Z_{N_a \times N_r}$) on polar form as seen in Fig.~\ref{fig:radar_polar_cart}.
 \begin{figure}
    \centering
    \includegraphics[width=\hsize]{Journal/figures/radar_method/polar_to_cartesian.png}
    \caption{Polar and Cartesian spinning radar data.}
    \label{fig:radar_polar_cart}
\end{figure}
Each row $a\in \{1..N_a\}$ and column $r\in\{1..N_r\}$ holds the reflected intensity and can be converted into Cartesian space:
\begin{equation}
%\begin{aligned}
\label{eq:cartesian}
    \mathbf{p} =
    \begin{bmatrix} p_x\\p_y
    \end{bmatrix}=
    \begin{bmatrix} d \gamma \text{cos}\left(\theta\right) \\ 
    d \gamma \text{sin}\left(\theta\right),
\end{bmatrix}
%&\mathcal{P}_f = \{\Mathbf{p}\}
%\end{aligned}
\end{equation}
where $\gamma$ is the range resolution of the radar and the azimuth angle $\theta$ can be computed via $\theta=2\pi a/m$.

The sensor has large max range with fine range resolution and operate largely unaffected by dust and all weather types. However, the data contain a large level of sensor specific noise including multi-path reflections, speckle noise and receiver saturation, therefor interpreting radar data e.g. for localization has been considered challenging.

We build on the radar filter ``$k$-strongest''~\cite{9636253} that efficiently computes a mask for further geometric analysis of areas around real landmarks. The method operates on azimuths individually by searching all $N_r$ range bins for the $k$ highest intensity values that additionally exceeds the expected noise level $z_{min}$. The noise level $z_{min}$ mitigates speckle noise and uncertain or false detections in absence of real obstacles. The limitation of $k$ returns per azimuth complements $z_{min}$ by mitigating multi-path reflections and receiver saturation under the assumption that true landmarks have higher intensity. 

While this method efficiently provides a course mask and generalize well across environment types, it does not accurately reconstruct the surface location and is unsuitable for accurately detecting small misalignment's. For that reason we propose an additional step aiming to further analyze masked regions and compute stable Radar Intensity Peak (RIP)-features. 
\subsection{Computation of Radar Intensity Peak (RIP)-features}
We aim to efficiently and accurately detect surface locations by finding peaks within masked regions where intensity is high over local neighbourhood.
For doing this, we combine non-maximum-suppression on 1D intensity-range signals together with a region strength criteria. For each range bin in the masked radar image, the region strength is computed as the average intensity in a window of size $w$. Second, we select all range bins where region strength exceeds neighbouring bins with the additional criteria that region strength must exceed the expected region noise floor. The algorithm is formally described in Alg.~\ref{alg:frip}. 
A typical behaviour is depicted in ~\ref{fig:radar_comparison}.
Structures such as buildings and vehicles appear with higher reflectively and produce more systematic

\begin{figure}
    \centering
    \includegraphics[width=\hsize,trim={2.7cm 3.1cm 10cm 4cm},clip]{Journal/figures/radar_method/filter_comparison.png}
    \caption{Sparse radar filtering presented in Cartesian space using the proposed method. The raw radar data (black-yellow) is first masked using ``k-strongest'' (cyan). Radar Intensity Peaks (RIP) features (black dots) are then extracted within masked regions.}
    \label{fig:radar_comparison}
\end{figure}


%We build upon the previous radar filtering technique $k-strongest$~\cite{9636253} that masks the polar radar image per by thresholding based on expected noise level $z_min$ and by additionally limit the nuber of returns to a maximum of $k$ per azimuth. This produces a mask that efficiently provides attention to the most important landmarks in the scene while discarding frequently occuring multipath reflections and less important secondary detections. 
%As an additional step, we use a peak detector that operate per azimuth on masked regions in the image together with non-maximum suppression.  

\newlength\myindent
\setlength\myindent{2em}
\newcommand\bindent{%
  \begingroup
  \setlength{\itemindent}{\myindent}
  \addtolength{\algorithmicindent}{\myindent}
}
\newcommand\eindent{\endgroup}

\begin{algorithm}
    \caption{RIP-Feature extraction}\label{alg:frip}
    \textbf{Input:} $Z_{N_a \times N_r}$ //Polar radar image\\
    \textbf{Parameters:} $w$ //window size\\ 
    \hspace{2cm} $k$ // $kstrongest$\\
    \hspace{2cm} $z_{min}$ // $kstrongest$\\
    \textbf{Output:} $\mathcal{F}_{rip}=\{(r,a)\}$ // set of range and angle tuples
    \begin{algorithmic}[1]
    \State $\mathcal{F}_{rip} \gets \emptyset$
    \For{$a \gets 1..N_a$ } //all azimuth bins
        %\State //Masking via $k-strongest$, subset of range bins
        \State $\mathcal{K} \gets kstrongest(\: Z(a,1..N_r),\: k,\: z_{min})$ %//bins of interest
        \State Initialize table \textbf{S} //Scores
        \For{$r \in \mathcal{K}\cup neighbours(\mathcal{K},w)$}
        \State $Scores[r]= 1/(2w+1)\sum_{n=r-2}^{r+2}  = Z(a,n)$ 
        \EndFor
        \For{$r \in \mathcal{K}$} //only search masked points
            \If{$\textbf{S}[r]>=max(\: neighbours(r,w)\: )$ }
                \If{$\textbf{S}[r] > z_{min}$ }
                    \State $\mathcal{F}_{rip} \gets \mathcal{F}_{rip} \cup \{(r,a)\}$
                \EndIf
            \EndIf
        \EndFor
    \EndFor
    \end{algorithmic}
\end{algorithm}
%begin{algorithm}
%\caption{An algorithm with caption}\label{alg:cap}
%\hspace*{\algorithmicindent} \textbf{Input:} $Z_{N_a \times N_r}$ \\
% \hspace*{\algorithmicindent} \textbf{Output} 
%\begin{algorithmic}
%\State asd
%\state input polar radar image $Z_{N_a \times N_r}$ 
%\State output a vector of range bins with landmarks
%\State $r$ \gets $k strongest(Z_{a, 1..N_r})$ %//vector of range bins
%\State $score$ is empty vector
%\State for each  {$i \in r $}
%\state $score_i$ = average intensity of window with size $w$\\
%\state peaks \gets peaks\\ %defined as all range bins which have scores larger than the score of their neighbours
%\end{algorithmic}
%\end{algorithm}

%FOR EACH AZIMUTH $a\in Z$
%$\mathcal{R}=Kstrongest(a)$ %get range bins with highest intensities
%$r \in R$
%for each remaining point in $p_r$,
%calculate the score by average intensity   $z_{mean}$ within a window of size $w=2$ neighbouring pixels in the raw radar image.
%$s_r =1/(window+1)\sum z_r$
%select all range bins where the score is higher than their closest neighbour and the score is higher than 

%%END FOR


==> Journal/related_work.tex <==
\label{sec:related_work}
 
Several methods have been used to assess alignment quality in the literature. However, in most cases these methods are used in an ad-hoc manner. Few systematic evaluations have been made of their general ability to be used as a classifier to detect aligned vs. misaligned point clouds. 

%\subsection{Alignment quality assessment for lidar point clouds}

One well-used alignment measure is the root-mean-squared (RMS) point-to-point distance, truncated by some outlier rejection threshold.  
This is also the function that is minimized by iterative closest point registration~\cite{icp}.
However, this measure has been shown to be highly sensitive to the environment and the choice of the outlier threshold \cite{silva-2005-ga,Almqvist} when trying to detect small errors. Consequently, this is a poor measure for alignment correctness classification.

One family of methods instead attempts to estimate the alignment uncertainty between point cloud pairs in the form of a covariance matrix~\cite{David_Landry,bengtsson_robot_2003,nieto_scan-slam_2006,prakhya_closed-form_2015}. 
Some use Monte Carlo strategies to estimate uncertainty by sampling registrations in a region \cite{bengtsson_robot_2003}. This exhaustive search is unpractical in mobile robotics.
Others attempt to estimate uncertainty in closed form using the Hessian \cite{censi-2007-accurate,magnusson-2009-phd,Almqvist}, representing the steepness of the alignment score function around a minimum. These methods assume that the registration has reached a global maximum, which is not necessarily true. 
Almqvist et al. include a covariance measure (NDT Hessian) in their evaluation which enables similar or less accuracy compared to RMS.
%Until today, alignment classification based on uncertainty covariance have been less accurate compared to matching score~\cite{Almqvist}.

Almqvist et al.~\cite{Almqvist} explored alignment classifiers based on RMS as well as other existing methods~\cite{rusinkiewicz-2001-fasticp,biber_normal_2003,magnusson-2009-phd,chandran-ramesh_assessing_2007,makadia-2006-fully,silva-2005-ga}, including the NDT score function~\cite{magnusson-2009-phd}, and investigated how to combine the measures with AdaBoost into a stronger classifier.
%
The classifiers were evaluated on two outdoor data sets, and although their classifiers reached almost 90\,\%  accuracy for the hardest cases on each data set individually, accuracy drops to around 80\,\% when cross-evaluating between the data sets.
In their evaluations, the NDT score function proved to be the best individual measure for alignment assessment. The combined AdaBoost classifier did not have significantly higher accuracy, but reduced parameter sensitivity. 
%our evaluation.

Liao et al. \cite{fuzzybnb} recently proposed a registration method based on fuzzy clusters, which involves a registration quality assessment. This fuzzy cluster-based quality assessment (FuzzyQA) compares the similarity of dispersion and disposition of points around fuzzy cluster centers. It has been used to detect if the point clouds are coarsely aligned, Coral instead attempts to detect small alignment errors.

Nobili et al.\cite{8462890} proposed a method to predict alignment risk prior to registration by combining overlap information and an alignment metric that quantifies the geometric constraints in the registration problem. Such alignment metric is based on point-to-plane residuals and has been evaluated in structured scenes with planar surfaces, while our method can operate well even in unstructured environments. Additionally, our method seeks to estimate the alignment after registration has been completed to introspectively measure the registration success, as opposed to predicting the risk prior to registration.


Bogoslavskyi et al.~\cite{Bogoslavskyi2017AnalyzingTQ} defined a quality metric based on positive and negative point information, and used it to measure alignment error and cluster three known object types in a controlled experiment. Rather than focusing on objects, our method aims to classify alignment quality of observed scenes in different environments. Additionally, their method operates on range images, which might not be available, while our method operates on unorganized point clouds.

To the best of our knowledge, there is no method for binary point cloud alignment classification that performs accurately and transfers well to new environments without parameter tuning or retraining.

%\subsection{Feature extraction and alignment quality using spinning radar}
Radar based methods that use alignment quality measures can be categorized into dense methods~\cite{barnes_masking_2020,Fourier_Mellin,9197231} that operate on raw radar images and do not explicitly perform data association, and sparse methods~\cite{hong2021radar,hong2020radarslam,burnett_we_2021,barnes_under_2020,burnett2021radar,8460687,8793990,kung2021normal,9636253} that compute alignment quality using key point locations, shape and descriptors over a correspondences set. Previous sparse methods use (weighted) Point-to-Point~\cite{barnes_under_2020,8460687,8793990}, Point-to-distribution~\cite{kung2021normal} and Point-to-Line~\cite{9636253} metrics. Key points can be extracted via SURF, blob detector~\cite{hong2021radar} gradient-based
feature detectors~\cite{8460687,8793990}, by a set of  oriented surface points~\cite{9636253} or distributions~\cite{kung2021normal} using a grid based approach, or by semi-supervised~\cite{barnes_under_2020} and unsupervised~\cite{barnes_under_2020,burnett2021radar} deep learning methods. 

While these methods for feature extraction and alignment quality have been used as objective functions for the purpose of estimating odometry, it is currently not known to which extent these metrics can be used for alignment correctness classification.
%Hence, we argue that existing learning-free feature extractors are able to compute consistent features in presence from challenging radar data.
Previous work shows that the performance of deep learning-based odometry methods decreases in new environment types~\cite{barnes_masking_2020,burnett_we_2021} however, methods have been succesfull in estimating odometry and perform SLAM in widely different environments without deep learning and even without parameter tuning~\cite{9636253,hong2021radar}. In this paper we show that learning-free feature extraction methods can produce stable key points over multiple environment types, and are suitable for alignment correctness classification in diverse environments. Hence we refrain from learning at the earlier steps to extracting features, but utilize learning first at a classification stage to find linear decision boundaries based on logistic regression.
